Quelques applications de l'Ansatz de Bethe (Some applications of the Bethe Ansatz)

The Bethe Ansatz is a method that is used in quantum integrable models in order to solve them explicitly. This method is explained here in a general framework, which applies to 1D quantum spin chains, 2D statistical lattice models (vertex models) and relativistic field theories with 1 space dimension and 1 time dimension. The connection with quantum groups is expounded. Several applications are then presented. Finite size corrections are calculated via two methods: The Non-Linear Integral Equations, which are applied to the study of the states of the affine Toda model with imaginary coupling, and their interpolation between the high energy (ultra-violet) and low energy (infra-red) regions; and the Thermodynamic Bethe Ansatz Equations, along with the associated Fusion Equations, which are used to determine the thermodynamic properties of the generalized multi-channel Kondo model. The latter is then studied in more detail, still using the Bethe Ansatz and quantum groups, so as to characterize the spectrum of the low energy excitations.

==> thesemac.tex <==
% macros pour ma these
%
\catcode`\@=11 % This allows us to modify PLAIN macros.
%
\edef\hyperdiese{\catcode`\noexpand\#=\the\catcode`\#}%%
\catcode`\#=12
\def\diese{#}%
\hyperdiese
\def\htmlhref#1#2{\special{html: <A href="#1">}#2%
\special{html: </A>}% place
}% un lien (texte #2 souligne) vers le label #1
\def\htmlname#1{\special{html: <A name="#1">}% place le label #1
}
%
\def\unred{\message{(This will come out unreduced.}%
\magnification=1200
\hsize=6.4truein\voffset=.1truein
%\hoffset=-.14truein\voffset=-.2truein
\baselineskip=16pt plus 2pt minus 1pt\footskip=13pt
\def\tfontsize{scaled\magstep3}}
%
\newdimen\fullhsize \newbox\leftpage \newdimen\hstitle \newdimen\hsbody
\newskip\footskip
\tolerance=1000\hfuzz=2pt\def\fontflag{cm}
\def\almostshipout#1{\if L\l@r \count1=1 \message{[\the\count0.\the\count1]}
      \global\setbox\leftpage=#1 \global\let\l@r=R
 \else \count1=2
  \shipout\vbox{\speclscape{\hsize\fullhsize\makeheadline}
      \hbox to\fullhsize{\box\leftpage\hfil#1}}  \global\let\l@r=L\fi}
%
\def\red{\message{(This will be reduced.} \let\l@r=L
\magnification=1000\baselineskip=12pt plus 1pt minus 1pt\footskip=11pt
\vsize=7truein
\def\tfontsize{scaled\magstep2}
\voffset=-.45truein\hoffset=-.75truein
\fullhsize=11.2truein\hsize=5.4truein
%
\output={
\almostshipout{\leftline{\vbox{\pagebody\makefootline}}}\advancepageno 
}}
\def\speclscape{\special{landscape}}
%
\font\footdigit=cmti7% at 6pt
%
%---------------------------------------------------------------------%
%
\def\bigans{b }
\ifx\answ\bigans\unred
%
\else\message{ big or little (b/l) }\read-1 to\answ
%
\ifx\answ\bigans\unred\else\red
\fi\fi
%---------------------------------------------------------------------
%
\newcount\yearltd\yearltd=\year\advance\yearltd by -1900
\def\Title#1#2{\nopagenumbers\abstractfont\rightline{#1}%
\vskip 1in\centerline{\titlefont #2}\abstractfont\vskip .5in}
%
\def\Date#1{\vfill\leftline{#1}\tenpoint\supereject}%
%
%       use following instead of \Date on the preliminary draft, 
%       puts date/time on each page in big mode, writes labels in margins
\def\draft{\draftmode\Date{\draftdate}}
\def\draftmode{\message{ DRAFTMODE }\def\draftdate{{\rm preliminary draft:
\number\month/\number\day/\number\yearltd\ \ \hourmin}}%
\headline={\hfil\draftdate}\writelabels
 {\count255=\time\divide\count255 by 60 \xdef\hourmin{\number\count255}
  \multiply\count255 by-60\advance\count255 by\time
  \xdef\hourmin{\hourmin:\ifnum\count255<10 0\fi\the\count255}}}
%       use \nolabels to get rid of eqn, ref, and fig labels in draft mode
\def\nolabels{\def\wrlabeL##1{}\def\eqlabeL##1{}\def\reflabeL##1{}}
\font\labfont=cmtt8 at 7pt
\def\writelabels{%
\def\wrlabeL##1{\hfill{\labfont\string##1}}
\def\eqlabeL##1{\hbox{\labfont\string##1}}
\def\reflabeL##1{{\noexpand\labfont\string\string\string##1}}
}
\nolabels
%
% tagged sec numbers
\global\newcount\chapno \global\chapno=0
\global\newcount\secno \global\secno=0
\global\newcount\meqno \global\meqno=1
%
\newif\iflongmess\longmessfalse
%
\def\newchap#1#2{\global\advance\chapno by1%
\message{(\the\chapno\iflongmess{. #2}\else\fi)}
\ifx\answ\bigans
\vfill\eject
\ifodd\the\pageno\else\ \vfill\eject\fi
\else \bigbreak\bigskip \fi
\global\secno=0\global\meqno=1
\xdef\chapsym{\the\chapno.}%
\htmlname{chapter.\the\chapno}%
\noindent{\titlefont\bf\chapsym\ #2}
%\headline{\hss\sl\chapsym\ #2\hss}
\writetoca{\htmlhref{\diese chapter.\the\chapno}{\chapsym\ #2}}
\DefWarn #1\xdef #1{\htmlhref{\diese chapter.\the\chapno}{{\bf\the\chapno}}}%
\writedef{#1\leftbracket#1}\wrlabeL#1
\par\nobreak\bigskip\nobreak}
%
\def\newnochap#1{%
\message{(\iflongmess{#1}\else\fi)}
\ifx\answ\bigans
\vfill\eject
\ifodd\the\pageno\else\ \vfill\eject\fi
\else \bigbreak\bigskip \fi
\global\secno=0\global\meqno=1
\xdef\chapsym{}
\htmlname{chapter.#1}%
\noindent{\titlefont\bf #1}
%\headline{\hss\sl #1\hss}
\writetoca{\htmlhref{\diese chapter.#1}{#1}}
\par\nobreak\bigskip\nobreak}
%
\def\newsec#1#2{\global\advance\secno by1%
\message{(\chapsym\the\secno\iflongmess{. #2}\else\fi)}
\bigbreak
\global\subsecno=0
\htmlname{section.\chapsym\the\secno}
\noindent{\bf\chapsym\the\secno. #2}
\writetoca{\string\quad
\htmlhref{\diese section.\chapsym\the\secno}{\chapsym\the\secno.\ #2}}
\DefWarn #1%
\xdef #1{\htmlhref{\diese section.\chapsym\the\secno}{{\bf\chapsym\the\secno}}}
\writedef{#1\leftbracket#1}\wrlabeL#1
\par\nobreak\medskip\nobreak}
%
\global\newcount\subsecno \global\subsecno=0
\def\subsec#1#2{\global\advance\subsecno by1
\message{(\chapsym\the\secno.\the\subsecno\iflongmess{. #2}\else\fi)}
\medbreak
\htmlname{subsection.\chapsym\the\secno.\the\subsecno}
\noindent{\it\chapsym\the\secno.\the\subsecno. #2}
\writetoca{\string\qquad
\htmlhref{\diese subsection.\chapsym\the\secno.\the\subsecno}
{\chapsym\the\secno.\the\subsecno.\ #2}}
\DefWarn #1
\xdef #1{\htmlhref{\diese subsection.\chapsym\the\secno.\the\subsecno}{{\it\chapsym\the\secno.\the\subsecno}}}
\writedef{#1\leftbracket#1}\wrlabeL#1
\par\nobreak\smallskip\nobreak}
%
%
%       $$a+b=c\eqn\label$$	gives displayed equation, numbered
%				consecutively within chapters.
%     
%
\def\eqn#1{
\eqno\htmlname{equation.\chapsym\the\meqno}(\chapsym\the\meqno)%
\eqlabeL#1%
\DefWarn #1\xdef #1{(\noexpand\htmlhref{\diese%pbl avec les dieses
equation.\chapsym\the\meqno}{\chapsym\the\meqno})}%
\writedef{#1\leftbracket#1}%
\global\advance\meqno by1}
\def\eqnalign#1#2{
\DefWarn #1%
% next line is to avoid bug with symbol #
\writedef{#1\leftbracket%
\immediate\write16{*** ERROR ... multiple eqn label \string\string\string#1\ 
cannot be called in advance ***}}%
%
\xdef#1##1{(\chapsym\the\meqno##1)\eqlabeL{#1\hskip.6mm ##1}}%
\eqalignno{%
\htmlname{equation.\chapsym\the\meqno}#2}%
\xdef#1##1{(\noexpand\htmlhref{\diese equation.\chapsym\the\meqno}%
{$\chapsym\the\meqno##1$})}%
\global\advance\meqno by1}
%
%			 footnotes
\def\footnotefont{\ninepoint}\def\f@t#1{\footnotefont #1\@foot}
\def\f@@t{\baselineskip\footskip\bgroup\footnotefont\aftergroup\@foot\let\next}
\setbox\strutbox=\hbox{\vrule height9.5pt depth4.5pt width0pt}
%
\global\newcount\ftno \global\ftno=0
\def\foot{\global\advance\ftno by1\footnote{$^{\hbox{\footdigit\the\ftno}}$}}
%
%say \footend to put footnotes at end
%will cause problems if \ref used inside \foot, instead use \nref before
\newwrite\ftfile
\def\footend{\def\foot{\global\advance\ftno by1\chardef\wfile=\ftfile
$^{\the\ftno}$\ifnum\ftno=1\immediate\openout\ftfile=foots.tmp\fi%
\immediate\write\ftfile{\noexpand\smallskip%
\noexpand\item{f\the\ftno:\ }\pctsign}\findarg}%
\def\footatend{\vfill\eject\immediate\closeout\ftfile{\parindent=20pt
\centerline{\bf Footnotes}\nobreak\bigskip\input foots.tmp }}}
\def\footatend{}
%
%     \ref\label{text}
% generates a number, assigns it to \label, generates an entry.
% To list the refs on a separate page,  \listrefs
%
\global\newcount\refno \global\refno=1
\newwrite\rfile
\global\newcount\citeno \global\citeno=1
%
\def\addpage#1{%
\expandafter\xdef\csname ref\expandafter\gobble\string#1\endcsname{%
\csname ref\expandafter\gobble\string#1\endcsname\ (\nobreak%
\htmlhref{\diese citation.\the\citeno}{p~\the\pageno}\nobreak)}%
\htmlname{citation.\the\citeno}%
\global\advance\citeno by1}%
\def\norefpages{\def\addpage##1{}}
%
\def\ref#1#2{\nref#1{#2}#1}
\def\nref#1#2{\DefWarn#1%
\xdef#1{\htmlhref{\diese reference.\the\refno}{\the\refno}% affiche numero
\noexpand\addpage\noexpand#1}% rajoute le numero de page a la fin de ref
\expandafter\xdef\csname ref\expandafter\gobble\string#1\endcsname{#2}%
\ifnum\refno=1\immediate\openout\rfile=refs.tmp\fi%
\chardef\wfile=\rfile\immediate%
\write\rfile{\noexpand\item{\reflabeL#1%
\htmlname{reference.\the\refno}[\the\refno]\ }%
\expandafter\string\csname ref\expandafter\gobble\string#1\endcsname%
\pctsign}%
\global\advance\refno by1}
%
\def\semi{;\hfil\break}
%
%\def\listrefs{\footatend\vfill\supereject\immediate\closeout\rfile\writestoppt
%\baselineskip=14pt
%\centerline{{\bf Références}}
%\bigskip{\frenchspacing%
%\parindent=20pt\input refs.tmp\vfill\eject}\nonfrenchspacing}
\def\listrefs{\footatend
\newnochap{Références}%
\immediate\closeout\rfile\writestoppt
\baselineskip=14pt
{\frenchspacing%
\parindent=20pt\input refs.tmp\vfill\eject}\nonfrenchspacing}
%
\def\startrefs#1{\immediate\openout\rfile=refs.tmp\refno=#1}
%
\def\refs#1{\count255=1[\r@fs #1{\hbox{}}]}
\def\r@fs#1{\ifx\und@fined#1\message{reflabel \string#1 is undefined.}%
\nref#1{need to supply reference \string#1.}\fi%
\vphantom{\hphantom{#1}}\edef\next{#1}\ifx\next\em@rk\def\next{}%
\else\ifx\next#1\ifodd\count255\relax\xref#1\count255=0\fi%
\else#1\count255=1\fi\let\next=\r@fs\fi\next}
%
%
\global\newcount\figno \global\figno=1
%
\input epsf
\def\epsfsize#1#2{#1}
\def\fig#1#2#3{%figure with just one eps picture
\figg#1{#2}{\centerline{\epsfbox{#3}}}}%
\long\def\figg#1#2#3{%
\DefWarn #1\xdef#1{\htmlhref{\diese figure.\the\figno}{\the\figno}}%
\writedef{#1\leftbracket #1}%
\midinsert%
\parindent=0pt\leftskip=1cm\rightskip=1cm\baselineskip=11pt%
\htmlname{figure.\the\figno}%
#3%
\vskip 8pt\ninepoint%
{\bf Fig.\ \the\figno:} #2\wrlabeL#1%\par
\endinsert%
\goodbreak%
\global\advance\figno by1%
}
%
\def\okeydokey{*}
\def\gobble#1{}
\def\DefWarn#1{%
\expandafter\if\csname tag\expandafter\gobble\string#1\endcsname\okeydokey%
\immediate\write16{*** WARNING ... the label \string#1 is already defined ***}%
\else%
\expandafter\xdef\csname tag\expandafter\gobble\string#1\endcsname{\okeydokey}%
\fi}
\def\label#1{%idee interessante mais buggee pour l'instant ...
\expandafter\if\csname tag\expandafter\gobble\string#1\endcsname\okeydokey%
#1\else%
\immediate\write16{*** WARNING ... the label \string#1 is undefined ***}%
\fi}
%
\newwrite\lfile
{\escapechar-1\xdef\pctsign{\string\%}\xdef\leftbracket{\string\{}
\xdef\rightbracket{\string\}}\xdef\numbersign{\string\#}}
\def\writedefs{\immediate\openout\lfile=labeldef.tmp%
\def\writedef##1{%
\immediate\write\lfile{\string\xdef\string##1\rightbracket}}}%
%
\def\writestop{\def\writestoppt{\immediate\write\lfile{\string\pageno%
\the\pageno\string\startrefs\leftbracket\the\refno\rightbracket%
\string\def\string\the\secno.\leftbracket\the\secno.\rightbracket%
\string\secno\the\secno\string\meqno\the\meqno}\immediate\closeout\lfile}}
%
\def\writestoppt{}\def\writedef#1{}
%
\newwrite\tfile \def\writetoca#1{}
\def\leaderfill{\leaders\hbox to 0.7em{\hss.\hss}\hfill}
%	use this to write file with table of contents
\def\writetoc{\immediate\openout\tfile=toc.tmp 
\def\writetoca##1{{\edef\next{\write\tfile{%
\noindent ##1   \string\leaderfill {\noexpand\number\pageno} \par}}\next}}}
%       and this lists table of contents on second pass
\def\listtoc{\centerline{\bf Table des matières}\nobreak\medskip{\baselineskip=12pt%
\parskip=0pt\catcode`\@=11%
\catcode`\#=12%
\input toc.tmp%
\hyperdiese%
\catcode`\@=12%
\bigbreak\bigskip}}
%
\def\readdefs{%
\catcode`\#=12%
\input labeldef.tmp%
\hyperdiese}%
%
\catcode`\@=12 % at signs are no longer letters
%
%	Unpleasantness in calling in abstract and title fonts
\font\titlerm=cmr10 \tfontsize \font\titlerms=cmr7 \tfontsize
\font\titlermss=cmr5 \tfontsize \font\titlei=cmmi10 \tfontsize
\font\titleis=cmmi7 \tfontsize \font\titleiss=cmmi5 \tfontsize
\font\titlesy=cmsy10 \tfontsize \font\titlesys=cmsy7 \tfontsize
\font\titlesyss=cmsy5 \tfontsize \font\titleit=cmti10 \tfontsize
\font\titlebf=cmbx10 \tfontsize
\skewchar\titlei='177 \skewchar\titleis='177 \skewchar\titleiss='177
\skewchar\titlesy='60 \skewchar\titlesys='60 \skewchar\titlesyss='60
%
\def\titlefont{\def\rm{\fam0\titlerm}% switch to title font
\textfont0=\titlerm \scriptfont0=\titlerms \scriptscriptfont0=\titlermss
\textfont1=\titlei \scriptfont1=\titleis \scriptscriptfont1=\titleiss
\textfont2=\titlesy \scriptfont2=\titlesys \scriptscriptfont2=\titlesyss
\textfont\itfam=\titleit \def\it{\fam\itfam\titleit}
\textfont\bffam=\titlebf \def\bf{\fam\bffam\titlebf}
\rm}
%
\font\authorfont=cmcsc10 \ifx\answ\bigans\else scaled\magstep1\fi
%
\ifx\answ\bigans\def\abstractfont{\tenpoint}\else
\font\abssl=cmsl10 scaled \magstep1
\font\absrm=cmr10 scaled\magstep1 \font\absrms=cmr7 scaled\magstep1
\font\absrmss=cmr5 scaled\magstep1 \font\absi=cmmi10 scaled\magstep1
\font\absis=cmmi7 scaled\magstep1 \font\absiss=cmmi5 scaled\magstep1
\font\abssy=cmsy10 scaled\magstep1 \font\abssys=cmsy7 scaled\magstep1
\font\abssyss=cmsy5 scaled\magstep1 \font\absbf=cmbx10 scaled\magstep1
\skewchar\absi='177 \skewchar\absis='177 \skewchar\absiss='177
\skewchar\abssy='60 \skewchar\abssys='60 \skewchar\abssyss='60
%
\def\abstractfont{\def\rm{\fam0\absrm}% switch to abstract font
\textfont0=\absrm \scriptfont0=\absrms \scriptscriptfont0=\absrmss
\textfont1=\absi \scriptfont1=\absis \scriptscriptfont1=\absiss
\textfont2=\abssy \scriptfont2=\abssys \scriptscriptfont2=\abssyss
\textfont\itfam=\bigit \def\it{\fam\itfam\bigit}\def\footnotefont{\tenpoint}%
\textfont\slfam=\abssl \def\sl{\fam\slfam\abssl}%
\textfont\bffam=\absbf \def\bf{\fam\bffam\absbf}\rm}\fi
%
\def\tenpoint{\def\rm{\fam0\tenrm}% switch back to 10-point type
\textfont0=\tenrm \scriptfont0=\sevenrm \scriptscriptfont0=\fiverm
\textfont1=\teni  \scriptfont1=\seveni  \scriptscriptfont1=\fivei
\textfont2=\tensy \scriptfont2=\sevensy \scriptscriptfont2=\fivesy
\textfont\itfam=\tenit \def\it{\fam\itfam\tenit}\def\footnotefont{\ninepoint}%
\textfont\bffam=\tenbf \def\bf{\fam\bffam\tenbf}\def\sl{\fam\slfam\tensl}\rm}
%
\font\ninerm=cmr9 \font\sixrm=cmr6 \font\ninei=cmmi9 \font\sixi=cmmi6 
\font\ninesy=cmsy9 \font\sixsy=cmsy6 \font\ninebf=cmbx9 
\font\nineit=cmti9 \font\ninesl=cmsl9 \skewchar\ninei='177
\skewchar\sixi='177 \skewchar\ninesy='60 \skewchar\sixsy='60 
%
\def\ninepoint{\def\rm{\fam0\ninerm}% switch to footnote font
\textfont0=\ninerm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
\textfont1=\ninei \scriptfont1=\sixi \scriptscriptfont1=\fivei
\textfont2=\ninesy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
\textfont\itfam=\ninei \def\it{\fam\itfam\nineit}\def\sl{\fam\slfam\ninesl}%
\textfont\bffam=\ninebf \def\bf{\fam\bffam\ninebf}\rm} 
%
%---------------------------------------------------------------------
%
\def\noblackbox{\overfullrule=0pt}
%
\def\inv{^{\raise.15ex\hbox{${\scriptscriptstyle -}$}\kern-.05em 1}}
\def\dup{^{\vphantom{1}}}
\def\Dsl{\,\raise.15ex\hbox{/}\mkern-13.5mu D} %this one can be subscripted
\def\dsl{\raise.15ex\hbox{/}\kern-.57em\partial}
\def\der{\partial}
\def\tr{{\rm tr}} \def\Tr{{\rm Tr}}
\font\bigit=cmti10 scaled \magstep1
\def\biglie{\hbox{\bigit\$}} %pound sterling
\def\lspace{\ifx\answ\bigans{}\else\qquad\fi}
\def\lbspace{\ifx\answ\bigans{}\else\hskip-.2in\fi} % $$\lbspace...$$
\def\boxeqn#1{\vcenter{\vbox{\hrule\hbox{\vrule\kern3pt\vbox{\kern3pt
	\hbox{${\displaystyle #1}$}\kern3pt}\kern3pt\vrule}\hrule}}}
\def\mbox#1#2{\vcenter{\hrule \hbox{\vrule height#2in
		\kern#1in \vrule} \hrule}}  %e.g. \mbox{.1}{.1}
%	matters of taste
%\def\tilde{\widetilde} \def\bar{\overline} \def\hat{\widehat}
%
% some sample definitions
\def\CAG{{\cal A/\cal G}} \def\CO{{\cal O}} %     curly letters
\def\CA{{\cal A}} \def\CC{{\cal C}} \def\CF{{\cal F}} \def\CG{{\cal G}} 
\def\CL{{\cal L}} \def\CH{{\cal H}} \def\CI{{\cal I}} \def\CU{{\cal U}}
\def\CB{{\cal B}} \def\CR{{\cal R}} \def\CD{{\cal D}} \def\CT{{\cal T}}
%\def\e#1{{\rm e}^{^{\textstyle#1}}}
\def\e#1{{\rm e}^{#1}}
\def\d{{\rm d}}
\def\grad#1{\,\nabla\!_{{#1}}\,}
\def\gradgrad#1#2{\,\nabla\!_{{#1}}\nabla\!_{{#2}}\,}
\def\ph{\varphi}
\def\psib{\bar\psi}
\def\om#1#2{\omega^{#1}{}_{#2}}
\def\vev#1{\langle #1 \rangle}
\def\lform{\hbox{$\sqcup$}\llap{\hbox{$\sqcap$}}}
\def\darr#1{\raise1.5ex\hbox{$\leftrightarrow$}\mkern-16.5mu #1}
\def\lie{\hbox{\it\$}} %pound sterling
\def\ha{{1\over2}}
\def\half{{\textstyle{1\over2}}} %puts a small half in a displayed eqn
\def\roughly#1{\raise.3ex\hbox{$#1$\kern-.75em\lower1ex\hbox{$\sim$}}}
\def\rhot{\tilde{\rho}}
\def\gs{{\rm g.s.}}
\def\eme#1{$#1^{\rm\grave eme}$}
\def\eps{\varepsilon}
\def\square{{\vcenter{
\hrule height.4pt
\hbox{\vrule width.4pt height4pt \kern4pt \vrule width.4pt\kern-0.5pt}
\hrule height.4pt
}}}
\def\squarea{{\vcenter{
\hrule height.4pt
\hbox{\vrule width.4pt height4pt \kern4pt \vrule width.4pt\kern-0.5pt}
\hrule height.4pt
\hbox{\vrule width.4pt height4pt \kern4pt \vrule width.4pt\kern-0.5pt}
\hrule height.4pt
}}}
\def\squares{{\vcenter{
\hrule height.4pt
\hbox{\vrule width.4pt height4pt \kern4pt \vrule width.4pt
\kern4pt \vrule width.4pt \kern-0.5pt}
\hrule height.4pt
}}}
\def\q#1{\lfloor #1\rfloor}
\def\qdim{q\dim}
\def\Matrix#1{\left(\matrix{#1}\right)}
\def\rep{rep}
\def\irr{irrep}
\def\cotan{\mathop{\rm cotan}\nolimits}
\def\mod{\ {\rm mod}\ }
\def\Im{\mathop{\rm Im}\nolimits}
%
\def\pre#1{{\tt[\htmlhref{http://xxx.lpthe.jussieu.fr/abs/#1}{\hbox{#1}}]}}
%
\font\tenmsb=msbm10
\font\sevenmsb=msbm7
\font\fivemsb=msbm5
\newfam\msbfam
\textfont\msbfam=\tenmsb
\scriptfont\msbfam=\sevenmsb
\scriptscriptfont\msbfam=\fivemsb
\def\Bbb{\fam\msbfam}
%
\font\teneuf=eufm10
\font\seveneuf=eufm7
\font\fiveeuf=eufm5
\newfam\euffam
\textfont\euffam=\teneuf
\scriptfont\euffam=\seveneuf
\scriptscriptfont\euffam=\fiveeuf
\def\goth{\fam\euffam}

